Transparent IFC Enforcement: Possibility and (In)Efficiency Results

Information Flow Control (IFC) is a collection of techniques for ensuring a no-write-down no-read-up style security policy known as noninterference. Traditional methods for both static and dynamic IFC suffer from untenable numbers of false alarms on real-world programs. Secure Multi-Execution (SME) promises to provide secure IFC without modifying the behaviour of already secure programs, a property known as transparency. Implementations of SME exist for the web and as plug-ins to several programming languages. Furthermore, SME can in theory work in a black-box manner, meaning that it can be programming language agnostic, making it perfect for securing legacy or third-party systems. As such SME, and its variants like Multiple Facets (MF) and Faceted Secure Multi-Execution (FSME), appear to be a family of panaceas for the security engineer. The question is, how come, given all these advantages, that these techniques are not ubiquitous in practice? The answer lies, partially, in the issue of runtime and memory overhead. SME and its variants are prohibitively expensive to deploy in many non-trivial situations. Why is this the case? On the surface, the reason is simple. The techniques in the SME family all rely on the idea of multi-execution, running all or parts of a program multiple times to achieve noninterference. Naturally, this causes overhead. However, the goal in the IFC community has been to overcome these overheads. In this paper we argue that there are fundamental reasons to expect this not to be possible and prove two key theorems: 1. All transparent enforcement is polynomial time equivalent to multi-execution. 2. All black-box enforcement takes time exponential in the number of principals in the security lattice. We also answer, in the affirmative, an open question about the possibility of transparently enforcing the TINI security condition.

==> level-assignment-restrictions.tex <==
In this section, we show that using level-assignments as an optimisation strategy
for multi-execution does not appear to be a promising technique.
%
This is worrying not just because enforcement boils down to computing level-assignments,
but also because all known methods for reducing exponential overhead to polynomial overhead
in multi-execution are based on some notion of level assignments.
%
Specifically, we show in Theorem \ref{thm:arbitrary-badness} that there are classes of
programs for which a naïve optimisation strategy produces arbitrarily bad results.
%
Furthermore, in Theorem \ref{thm:no-minimal} we show that no reasonable level assignment
can be minimal.
%

\begin{definition}[Minimal Level Assignment]
  $L$ is minimal for the subset $\mathbb{L}$ of all level assignments if for
  any other level assignment $L' \in \mathbb{L}$ we have that if $L$ and $L'$ terminate
  on $p, x$ we have that $|L(p, x)| \le |L'(p, x)|$.
\end{definition}

\begin{lemma}
  \label{lemma:minimal-emptyset}
  If $L$ is a minimal \TX-$\TX'$ level assignment and $L$ terminates on $p, x$ where
  $p$ is not \TX'-secure, then $L(p, x) = \emptyset$.
\end{lemma}
\begin{proof}
  Assume this is not the case, i.e. there are $p, x$ where $p$ is not \TX'-secure
  such that $|L(p, x)| > 0$.
  %
  Define $L'$ as:
  %
  $$
  L'(q, x) =
  \begin{cases}
    &\emptyset\ \text{if}\ p = q\\
    &L(q, x)\ \text{otherwise}
  \end{cases}
  $$
  %
  Note that $L'$ is a \TX-$\TX'$ level assignment, but $|L'(p, x)| < |L(p, x)|$.
  %
  This is a contradiction, so if $L$ terminates on $p, x$ then $L(p, x) = \emptyset$.
\end{proof}

\begin{theorem}[No Minimal Level Assignments]
  \label{thm:no-minimal}
  There is no minimal \TI-\Total~level assignment.
\end{theorem}
\begin{proof}
  Assume such a level assignment $L$ exists for the two-point lattice.
  %
  Observe that Turing Machine (TM) totality is not semi-decidable \cite{rogers1967theory}.
  %
  Given a TM $M$, define:
  $$
  \sem{p_M}(x) =
    \begin{cases}
      &\udef\ \text{if}\ M\ \text{terminates on tape}\ |x|\\
      &\{\sem{M}(|x|)^{\color{red} H}\}\ \text{otherwise}
    \end{cases}
  $$
  %
  Note that $p_M$ is \Total-secure if and only if $M$ is total.
  %
  If $p_M$ is not \Total-secure, then either $L(p, \emptyset)$ diverges
  or $L(p, \emptyset) = \emptyset$ as $L$ is minimal.
  %
  If $p_M$ is \Total-secure, then $\defined{L}{p, x}$ and
  by Lemma \ref{lemma:minimal-emptyset} also $L(p, \emptyset) = \{{\color{red} H}\}$.
  %
  This gives us a semi-decision proceedure for TM-totality, which is a contradiction.
\end{proof}

Postulate a minimal level assignment $L_{\text{\TX-\Total-best}}$ for the set of \TX-\Total~
level assignments.
%
Clearly, $L_{\text{\TX-\Total-best}}$ can not be implemented.
%
However, we can use it to guage the potential overhead introduced by
a level assignment.

\begin{theorem}[Arbitrary Badness]
  \label{thm:arbitrary-badness}
  %
  Assume $\L = \Pow{A}$ for some non-finite $A$.
  %
  Given any $N \in \Nat$ we have for any \TX-\Total~level assignment $L$,
  there exists a program $p$ and input $x$ such that $|L_{\text{\TX-\Total-best}}(p,x)| = 0$
  and $|L(p, x)| \ge N$.
\end{theorem}
\begin{proof}
  Assume this was not the case.
  %
  Define $A_N = \{a_i\ |\ i \in [1, N] \}$ where $a_i = a_j$ if and
  only if $i = j$.
  %
  Given a Turing Machine $M$ define $p_M$ as:
  %
  $$
  \sem{p_M}(x) =
  \begin{cases}
    &\udef\ \text{if}\ M\ \text{diverges on}\ |x\project\bot|\\
    &\{ \sem{M}(x\project\bot)^{\{a\}}\ |\ a \in A_N \}\ \text{otherwise}
  \end{cases}
  $$
  %
  Note that $p_M$ is \Total-secure if and only if $M$ is total.
  %
  If $|L(p_M, \emptyset)| < N$ or $L$ diverges, we know that $p_M$ is not
  \Total-secure, as the semantics of $p_M$ are not preserved by $L$ should
  $p_M(\emptyset)$ be defined.
  %
  As $L(p_M, \emptyset)$ is no more than $N-1$ elements larger than
  $|L_{\TX-\Total-\text{best}}(p, \emptyset)$, if $|L(p_M, \emptyset)| \ge N$
  we know that $L_{\TX-\Total-\text{best}}(p, A_N) \not= \emptyset$
  and so $p_M$ must be \Total-secure, meaning that $M$ is total.
  %
  In other words, by computing $|L(p_M, \emptyset)| \ge N$ we obtain
  a semi decision proceedure for Turing Machine totality, which is impossible
  \cite{rogers1967theory}.
\end{proof}

